Fine tuning Pre trained Models for Robustness Under Noisy Labels

The presence of noisy labels in a training dataset can significantly impact the performance of machine learning models. To tackle this issue, researchers have explored methods for Learning with Noisy Labels to identify clean samples and reduce the influence of noisy labels. However, constraining the influence of a certain portion of the training dataset can result in a reduction in overall generalization performance. To alleviate this, recent studies have considered the careful utilization of noisy labels by leveraging huge computational resources. Therefore, the increasing training cost necessitates a reevaluation of efficiency. In other areas of research, there has been a focus on developing fine-tuning techniques for large pre-trained models that aim to achieve both high generalization performance and efficiency. However, these methods have mainly concentrated on clean datasets, and there has been limited exploration of the noisy label scenario. In this research, our aim is to find an appropriate way to fine-tune pre-trained models for noisy labeled datasets. To achieve this goal, we investigate the characteristics of pre-trained models when they encounter noisy datasets. Through empirical analysis, we introduce a novel algorithm called TURN, which robustly and efficiently transfers the prior knowledge of pre-trained models. The algorithm consists of two main steps: (1) independently tuning the linear classifier to protect the feature extractor from being distorted by noisy labels, and (2) reducing the noisy label ratio and fine-tuning the entire model based on the noise-reduced dataset to adapt it to the target dataset. The proposed algorithm has been extensively tested and demonstrates efficient yet improved denoising performance on various benchmarks compared to previous methods.

==> command/checklist.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> command/impact.tex <==
\newpage
\section*{Broader Impact and Limitation}

Our research investigates the utilization of high-quality pre-trained models for datasets with noisy labels. The proposed algorithm is strongly motivated by two key observations: (1) When pre-trained models can generate well-defined class-wise clusters, fine-tuning the entire set of trainable parameters yields better results than linear probing. (2) In cases where pre-trained models fail to generate sufficiently accurate clusters, tuning through linear probing shows promise. This study builds upon and extends previous findings~\cite{cheng2023mitigating}, combining the strengths of both linear probing (LP) and full fine-tuning (FFT) methods.

However, there are certain limitations to our observations and experimental results. Firstly, our focus is restricted to only two types of tuning methods, LP and FFT. Secondly, our research is limited to classification tasks, and it is essential to extend our findings to other tuning methods and different tasks such as object detection or segmentation. Additionally, the use of pre-trained models often requires substantial computational resources. Although our approach attempts to reduce the training time and computational costs, the underlying reason for their resource-intensive nature lies in the large model size. This implies that measures to decrease memory requirements need to be explored, including strategies such as adjusting the batch size to alleviate the computational burden.



==> src/fig/03_pretraining.tex <==
\begin{figure*}
    \begin{minipage}{.49\textwidth}
        \centering
            \begin{subfigure}{0.49\textwidth}
                    \includegraphics[width=1.\linewidth]{src/fig_src/tsne_cifar10.pdf}
                    \caption{t-SNE CIFAR-10}
                    \label{fig:tsne_c10}
            \end{subfigure}
            \begin{subfigure}{0.49\textwidth}
                    \includegraphics[width=1.\linewidth]{src/fig_src/cifar10_clean.pdf}
                    \caption{CIFAR-10 Cleansing}
                    \label{fig:f1}
            \end{subfigure}
    \caption{CIFAR-10 analysis: (a) t-SNE~\cite{van2008visualizing} plot and (b) noisy label cleansing performance through linear probing. It shows well-clustering and sufficient cleansing performance for all classes.}
    \label{fig:cifar10_anal}
    \end{minipage}
    \hfill
    \begin{minipage}{.49\textwidth}
            \begin{subfigure}{0.49\textwidth}
                    \includegraphics[width=1.\linewidth]{src/fig_src/tsne_cifar100.pdf}
                    \caption{t-SNE CIFAR-100}
                    \label{fig:tsne_c100}
            \end{subfigure}
            \begin{subfigure}{0.49\textwidth}
                    \includegraphics[width=1.\linewidth]{src/fig_src/cifar100_clean.pdf}
                    \caption{CIFAR-100 Cleansing}
                    \label{fig:f1_out}
            \end{subfigure}
    \caption{CIFAR-100 analysis: (a) t-SNE~\cite{van2008visualizing} plot and (b) noisy label cleansing performance through linear probing. It shows there exists some classes are difficult to be well-clustered and cleansed.}
    \label{fig:cifar100_anal}
    \end{minipage}
\vspace{-5pt}
\end{figure*}

% \begin{figure*}
%     \begin{minipage}{.495\textwidth}
%         \hfill
%         \begin{subfigure}{0.235\textwidth}
%                 \includegraphics[width=1.\linewidth]{src/fig_src/tsne_cifar100.pdf}
%                 \caption{t-SNE CIFAR-100}
%                 \label{fig:tsne_c100}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.235\textwidth}
%                 \includegraphics[width=1.\linewidth]{src/fig_src/cifar100_f1.pdf}
%                 \caption{$F_1$ score CIFAR-100}
%                 \label{fig:f1_out}
%         \end{subfigure}
%     \end{minipage}
%     \caption{
%     The motivation of \alg. (a), (b): t-SNE\,\cite{van2008visualizing} for 10 randomly selected classes of CIFAR-10/100 datasets. (c): Comparison of $F_1$ scores on various noise distributions of CIFAR-10. (d) Comparison of $F_1$ scores for familiar and unfamiliar classes on various noise distributions of CIFAR-100. \alg exhibits exceptional performance in identifying instances with noisy labels among familiar classes when trained on the either true (ELR) or corrupted (CE) conditional distribution. However, it is hard to extend this success to unfamiliar classes.
%     % For familiar classes, \alg demonstrates strong performance in identifying noisy labels in both cases for sufficiently trained on true\,(ELR) and corrupted\,(CE) conditional distribution (especially for true distribution), however, it struggles with unfamiliar classes. 
%     }
% \end{figure*}

==> src/fig/app_imgs.tex <==
\begin{figure*}
    \centering
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=1.\linewidth]{src/fig_src/imgnet.pdf}
                \caption{ImageNet}
                \label{fig:imgnet}
        \end{subfigure}
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=1.\linewidth]{src/fig_src/cifar.pdf}
                \caption{CIFAR}
                \label{fig:cifar}
        \end{subfigure}
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=1.\linewidth]{src/fig_src/eurosat.pdf}
                \caption{EuroSAT}
                \label{fig:eurosat}
        \end{subfigure}            
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=1.\linewidth]{src/fig_src/dtd.pdf}
                \caption{DTD}
                \label{fig:dtd}
        \end{subfigure}            
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=1.\linewidth]{src/fig_src/pet.pdf}
                \caption{Oxford-IIIT Pet}
                \label{fig:pet}
        \end{subfigure}                        
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=1.\linewidth]{src/fig_src/clothing1m.pdf}
                \caption{Clothing1M}
                \label{fig:clothing1m}
        \end{subfigure}
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=1.\linewidth]{src/fig_src/webvision.pdf}
                \caption{WebVision}
                \label{fig:webvision}
        \end{subfigure}
    \caption{Example Images for each dataset.}
    \label{fig:imgs}
        
\end{figure*}
